NeRF-RPN: A general framework for object detection in NeRFs

This paper presents the first significant object detection framework, NeRF-RPN, which directly operates on NeRF. Given a pre-trained NeRF model, NeRF-RPN aims to detect all bounding boxes of objects in a scene. By exploiting a novel voxel representation that incorporates multi-scale 3D neural volumetric features, we demonstrate it is possible to regress the 3D bounding boxes of objects in NeRF directly without rendering the NeRF at any viewpoint. NeRF-RPN is a general framework and can be applied to detect objects without class labels. We experimented NeRF-RPN with various backbone architectures, RPN head designs and loss functions. All of them can be trained in an end-to-end manner to estimate high quality 3D bounding boxes. To facilitate future research in object detection for NeRF, we built a new benchmark dataset which consists of both synthetic and real-world data with careful labeling and clean up. Code and dataset are available at https://github.com/lyclyc52/NeRF_RPN.

==> 6_applications.tex <==
%\section{Applications}
%\subsection{3D Object Detection}
% \vspace{1mm}
% \noindent\textbf{Application: Scene Editing} We can edit the scene in NeRF given the proposals produced by our NeRF-RPN. See Figure~\ref{fig:edit} for a demonstration which sets the volume density inside the proposal bounding box to zero before rendering the image.
% \input{figs/fig-scene_editing.tex}


%

% \subsection{robot map}


==> figs/fig-head.tex <==
\begin{figure}[t]
    \subfloat[Anchor-based 3D RPN Head]{%
      \includegraphics[clip,width=1\columnwidth]{figs/rpn_head1.pdf}%
      \label{fig:head_a}
    }
    \vspace{0.15in}
    
    \subfloat[Anchor-free 3D RPN Head]{%
      \includegraphics[clip,width=1\columnwidth]{figs/rpn_head2.pdf}%
      \label{fig:head_b}
    }
    \caption{\textbf{3D RPN Heads.} }
    \label{fig:head}
    
\end{figure}

% \begin{figure}[t]
%     \includegraphics[width=1\linewidth]{figs/rpn_head.pdf}
%     \caption{\textbf{RPN Head.} }
%     \label{fig:head}
%     % \vspace{-0.1in}
% \end{figure}

==> figs/fig-midpoint.tex <==
\begin{figure}[t]
    \subfloat[Anchor-based bounding box representation]{%
      \includegraphics[clip,width=1\columnwidth]{figs/midpoint_coder1.pdf}%
      \label{fig:midpoint_a}
    }
    \vspace{0.15in}
    
    \subfloat[Anchor-free bounding box representation]{%
      \includegraphics[clip,width=1\columnwidth]{figs/midpoint_coder2.pdf}%
      \label{fig:midpoint_b}
    }
    \caption{\textbf{3D Midpoint Offset Bounding Box Representations.} }
    \label{fig:midpoint}
    
\end{figure}

==> figs/fig-rebuttal-qualitative.tex <==
\newcommand\width{0.00cm}
\newcommand\height{0.01cm}
\newcommand{\gt}{Ground truth}
\newcommand{\ours}{Ours}
\newcommand{\imvoxelnet}{ImVoxelNet}
\newcommand{\fcaf}{FCAF3D}

%\newcommand{\img1}[]{}

\begin{figure}[ht]
    \centering
    \captionsetup[subfloat]{labelformat=empty}

    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/gt/ai_001_006_0017.png}}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/imvoxelnet/ai_001_006_0017_resize.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/fcaf3d/ai_001_006_0017_resize.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/nerf_rpn/ai_001_006_0017_resize.png}}
	
    \vspace{\height}

    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/gt/ai_022_005_frame.0001.tonemap.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/imvoxelnet/ai_022_005_frame.0001.tonemap_resize.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/fcaf3d/ai_022_005_0001_resize.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/nerf_rpn/ai_022_005_0001_resize.png}}
	
    \vspace{\height}

    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/gt/3dfront_0004_00_04.png}}\hspace{\width}
	\subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/imvoxelnet/3dfront_0004_00_04.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/fcaf3d/3dfront_0004_00_04.png}}\hspace{\width}
    \subfloat{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/nerf_rpn/3dfront_0004_00_04.png}}
	
    \vspace{\height}
 
    \subfloat[\gt]{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/gt/3dfront_0075_01_0009.png}}\hspace{\width}
    \subfloat[\imvoxelnet]{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/imvoxelnet/3dfront_0075_01_0009.png}}\hspace{\width}
    \subfloat[\fcaf]{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/fcaf3d/3dfront_0075_01_09.png}}\hspace{\width}
    \subfloat[\ours]{\includegraphics[width = 0.24\linewidth]{figs/rebuttal/nerf_rpn/3dfront_0075_01_0009.png}}
	
    \vspace{-0.1in}
    \caption{\textbf{Qualitative Results.} Row 1 \& 2: Hypersim. Row 3 \& 4: 3D-FRONT.}
    \vspace{-0.2in}
    \label{fig:rebuttal-qualitative}
\end{figure}

==> tabs/tab-mask.tex <==
\begin{table}[t]
\footnotesize
\newcommand{\xpm}[1]{{\tiny$\pm#1$}}
% \setlength{\tabcolsep}{5pt}
\centering % \footnotesize
% \resizebox{0.47\textwidth}{!}{
\begin{tabular}{lccc}

\toprule
  Method    & before refinement     & before refinement   & \\ \midrule
  Mask IoU $\uparrow$  & $\mathbf{0.86}$ & $\mathbf{0.76}$  \\ 

\bottomrule



% \toprule
%   Method        & Mask IoU $\uparrow$ & \\ \midrule
%   before refinement          & $\mathbf{0.86}$  \\ \midrule 

%   before refinement   & $\mathbf{0.76}$ \\ 

% \bottomrule
\end{tabular}
% }
\caption{\textbf{Masks comparison.} We evaluate the IoU errors of all objects over the 8 scenes before and after the refinement step.}
\label{tab:mask}
\vspace{-0.5em}
\end{table}


==> tabs/tab-rebuttal-quan.tex <==
\begin{table}[]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lllllllllllll}
\hline
\multirow{2}{*}{Methods} & \multicolumn{4}{c}{Hypersim} & \multicolumn{4}{c}{3D-FRONT} & \multicolumn{4}{c}{ScanNet} \\
 & AR25 & AR50 & AP25 & AP50 & AR25 & AR50 & AP25 & AP50 & AR25 & AR50 & AP25 & AP50 \\ \hline
ImVoxelNet & 19.7 & 5.7 & 9.7 & 2.3 & 88.3 & 71.5 & \textbf{86.1} & \textbf{66.4} & 51.7 & 20.2 & 37.3 & 9.8 \\
FCAF3D & 47.6 & 19.4 & 30.7 & 8.8 & 89.1 & 56.9 & 73.1 & 35.2 & \textbf{90.2} & 42.4 & \textbf{63.7} & \textbf{18.5} \\ \hline \hline
Ours (anchor-based) & 57.1 & 14.9 & 11.2 & 1.3 & \textbf{97.8} & \textbf{76.5} & 65.9 & 43.2 & 88.7 & 42.4 & 40.7 & 14.4 \\
Ours (anchor-free) & \textbf{66.7} & \textbf{27.3} & \textbf{30.9} & \textbf{11.5} & 96.3 & 69.9 & 85.2 & 59.9 & 89.2 & \textbf{42.9} & 55.5 & 18.4 \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\caption{\textbf{Comparisons.} Our methods use VGG19.}
\vspace{-0.2in}
\label{tab:rebuttal_quan}
\end{table}
